Open-source Stand-Alone Versatile Tensor Accelerator

Machine Learning (ML) applications demand significant computational resources, posing challenges for safety-critical domains like aeronautics. The Versatile Tensor Accelerator (VTA) is a promising FPGA-based solution, but its adoption was hindered by its dependency on the TVM compiler and by other code non-compliant with certification requirements. This paper presents an open-source, standalone Python compiler pipeline for the VTA, developed from scratch and designed with certification requirements, modularity, and extensibility in mind. The compiler's effectiveness is demonstrated by compiling and executing LeNet-5 Convolutional Neural Network (CNN) using the VTA simulators, and preliminary results indicate a strong potential for scaling its capabilities to larger CNN architectures. All contributions are publicly available.

==> extended_abstract.tex <==
\section{Extended abstract}
Embedding Machine Learning (ML) applications in safety-critical systems, particularly in aeronautics, is gaining increasing interest due to the significant benefits it offers for complex tasks such as object recognition and speech-to-text. 
However, executing these ML models requires intensive computations, and current avionic hardware cannot offer sufficient capacity.
Dedicated accelerators, such as the Versatile Tensor Accelerator (VTA), are promising hardware candidates for such applications. 
The VTA strikes an effective balance between performance and power consumption. 
For instance, Daedalean has developed vision-based functions for aircraft based on Convolutional Neural Networks (CNNs) using VTA-inspired accelerators.

The VTA is an open-source hardware accelerator proposed by TVM to efficiently execute matrix multiplications which are the key operation for any CNN.
In addition to the hardware accelerator, the VTA comes with both a functional simulator written in C++ and a Register-Transfer Level (RTL) hardware description via CHISEL.
The C++ simulator takes the same binary instructions and binary data as the FPGA implementation and returns the result. 
This allows visualisation and analysis of the values computed by the VTA for any matrix multiplication.
The CHISEL simulator goes further by providing cycle-accurate simulations, enabling the tracking of operations, memory states, and memory transactions at each cycle.

Despite its advantages, the VTA faces significant limitations that hinder its broader adoption. First, the VTA is no longer maintained as TVM has phased it out. 
Second, the use of the VTA and its simulators is not unified. 
Indeed, the CHISEL simulator accepts a JSON file, whereas the other two accept raw binary files.
Third, the cycle-accurate simulation only provides a test environment for some specific submodules, not the entire VTA architecture. 
Fourth, the VTA compiler is intricated in the TVM compiler making it complex to be certified.

To address these issues, we propose four main contributions. 
First, we will create a stand-alone VTA GitHub repository to maintain the VTA alive. 
For example, the CHISEL description was based on CHISEL version 3.5, which is outdated and incompatible with modern frameworks like chiseltest. 
Second, we will unify the functional (C++) and cycle-accurate (CHISEL) simulation approaches by using the same binaries as the accelerator itself as input. 
Third, we will enrich the cycle-accurate simulation to run tests on different submodules and provide multiple available tests. 
Thanks to this capacity, we will be able to evaluate and compare different implementations of the same operation. The purpose being to assess the number of cycles and memory size.
Fourth, we will develop an open-source VTA compiler that operates independently of TVM, making a step towards improving the VTA's applicability in aeronautics. 

If accepted, the final paper will present a new open-source stand-alone GitHub repository designed to address the issues outlined earlier. To start, we will provide a detailed overview of the VTA architecture, which consists of three main parallel modules: Load, Compute, and Store. These modules work together to provide efficient data computation.
The Compute module is central to the VTA operation and is further divided into two submodules: TensorGemm, responsible for matrix multiplications, and TensorAlu, which handles element-wise operations (e.g., ReLU – Rectified Linear Unit). We will explain how these submodules are designed to handle these operations, describing how instructions are encoded and executed within the accelerator.
These insights will be supported by practical simulation examples.
For example, the Compute module can multiply two 16-by-16 element matrices in just 3 instructions and 32 cycles, while multiplying two 32-by-32 element matrices requires 3 instructions and 146 cycles. 
In addition, to illustrate the performance and capabilities of these modules, we will present simulations of well-known CNNs, such as LeNet-5.
Lastly, we will introduce a stand-alone Python-based compiler that is capable of decomposing larger matrices into the required shapes, arranging them for efficient data mapping, and specifying the sequence of instructions for the VTA to execute. The compilation process will be explained in depth, using examples generated from simulations to demonstrate the full workflow.

In conclusion, this work provides: a comprehensive update to the VTA ecosystem, addressing its maintenance issues; a unified simulation interface for both the functional and cycle-accurate simulators; an enriched cycle-accurate simulation with examples; and an open-source compiler to generate the binaries necessary for both the simulation and the FPGA implementation. All these contributions will be made available in a dedicated GitHub repository.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

